How Adults Understand What Young Children Say

Children's early speech often bears little resemblance to that of adults, and yet parents and other caregivers are able to interpret that speech and react accordingly. Here we investigate how these adult inferences as listeners reflect sophisticated beliefs about what children are trying to communicate, as well as how children are likely to pronounce words. Using a Bayesian framework for modeling spoken word recognition, we find that computational models can replicate adult interpretations of children's speech only when they include strong, context-specific prior expectations about the messages that children will want to communicate. This points to a critical role of adult cognitive processes in supporting early communication and reveals how children can actively prompt adults to take actions on their behalf even when they have only a nascent understanding of the adult language. We discuss the wide-ranging implications of the powerful listening capabilities of adults for theories of first language acquisition.

==> CDL (Arxiv revision 2)/tables/model_surprisal_comparison.tex <==
\begin{table*}
\caption{Average prior and posterior surprisal and rank of transcriber interpretations on $n = 43,993$ phonetic sequences for sixteen Bayesian spoken word recognition models.
This set reflects crossing eight priors with two likelihoods. 
Lower surprisal and lower rank both indicate a closer match to adult listeners.}

 

\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|ll|ll|ll}
                 & \multicolumn{2}{c|}{Prior} & \multicolumn{2}{c|}{Posterior with WFST Likelihood} & \multicolumn{2}{c}{Posterior with Lev. Dist. Likelihood} \\
\cline{2-7}
                 & Average     & Average       & Average       & Average    & Average       & Average    \\
                 & Surprisal$^\star$     & Rank$^\ddagger$       & Surprisal$^\star$       & Rank$^\ddagger$ & Surprisal$^\star$       & Rank$^\ddagger$        \\
Language Model Prior             & (bits$^\dagger$)        &        & (bits$^\dagger$)          & & (bits$^\dagger$)          &         \\ \hline
\textsc{CDL+Context} & 3.30          & 50.21      & 0.63            & 2.41 & 1.15 & 7.89  \\
\textsc{Switchboard+Context} & 4.10          & 110.46      & 0.85            & 4.61 &  1.52  & 13.95       \\
\textsc{BERT+Context}     & 4.63          & 140.99     & 1.02            & 6.16     & 1.69   & 18.52   \\
\textsc{CDL+OneUtt}  & 5.06          & 124.31     & 1.09            & 7.39   & 1.90 & 23.37\\
\textsc{Switchboard+OneUtt}  & 6.46          & 362.90     & 1.52            & 15.19 & 2.62& 45.06\\
\textsc{BERT+OneUtt}      & 7.35          & 494.18     & 1.81            & 17.34     &  2.53 & 42.93 \\
\textsc{CHILDES-1gram}   & 8.79          & 314.09     & 2.26            & 15.89     &  3.76 & 49.00 \\
\textsc{UniformPrior}    & 12.97         & 3998.00       & 4.61            & 62.50 & 4.87 & 138.31 
\end{tabular}
\end{center}
\footnotesize{\noindent $^\star$ The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ Ranks are taken out of a vocabulary of 7,997 possible words.}
\end{table*}

==> CDL (Arxiv revision 2)/tables/model_surprisal_comparison2.tex <==
\begin{table*}
\tablefont
\caption{Model performance as measured by average surprisal, average rank of transcriber interpretation, and percentage of correct top guesses for word recognition models.
The  left column (``Prior'') reflects the distributions from the word prediction module, \ie before using the child's production to identify the word.
The center and right columns reflect the distributions after integrating information from two variants of the pronunciation module.
The full model is indicated in red, which we expect to best replicate adult interpretations of child speech.
This is the best performing model, as indicated in bold.
Other models represent ablations with respect to this full model. 
%Average surprisal measures the average negative log probability that the model assigns to the words found by transcribers; lower indicates a closer match to adult listeners.
%Average rank indicates the rank of the transcriber's interpretation among the model's hypotheses  (lower is better, e.g., rank = 2 means that it was the second most probable interpretation under the model).
%Percent top 1-guess is the proportion of words in the test set where the model assigns the highest probability among all words in the vocabulary to the word found by annotators; higher is better.
}
\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|lll||lll|lll}
                 & \multicolumn{3}{c||}{Prior} & \multicolumn{3}{c|}{Posterior with WFST Likelihood} & \multicolumn{3}{c}{Posterior with Lev. Dist. Likelihood} \\
\cline{2-10}
                 & Average     & Average       & Correct       & Average    & Average       & Correct & Average  & Average & Correct  \\
                 & Surprisal$^\star$     & Rank$^\ddagger$       &
                 Top  & Surprisal$^\star$       & Rank$^\ddagger$ &
                 Top &
                 Surprisal$^\star$       & Rank$^\ddagger$ & Top       \\
Language Model Prior             & (bits$^\dagger$)        &    &  Guess  & (bits$^\dagger$) &         &  Guess & (bits$^\dagger$)          &      &  Guess \\ \hline
& & & & \multicolumn{3}{c|}{\cellcolor{red!25} Full Model} & \multicolumn{3}{c}{\cellcolor{blue!25} Ablated Models}    \\
\textsc{CDL+Context} & 3.30          & 50.21 & 55\%       & \cellcolor{red!25} \textbf{0.63}            & \cellcolor{red!25}\textbf{2.41} & \cellcolor{red!25} \textbf{90\%} & \cellcolor{blue!25} 1.15 & \cellcolor{blue!25} 7.89 & \cellcolor{blue!25} 83\%  \\
\textsc{Switchboard+Context} & 4.10          & 110.46   & 49\%   & \cellcolor{blue!25} 0.85            & \cellcolor{blue!25} 4.61 & \cellcolor{blue!25}87\% &  \cellcolor{blue!25} 1.52  & \cellcolor{blue!25}13.95  & \cellcolor{blue!25} 78\%     \\
\textsc{BERT+Context}     & 4.63          & 140.99    & 45\%  & \cellcolor{blue!25} 1.02            & \cellcolor{blue!25} 6.16  & \cellcolor{blue!25} 84\%   & \cellcolor{blue!25} 1.69   & \cellcolor{blue!25} 18.52 & \cellcolor{blue!25} 76\%  \\
\textsc{CDL+OneUtt}  & 5.06          & 124.31  & 36\%   & \cellcolor{blue!25} 1.09            & \cellcolor{blue!25} 7.39 & \cellcolor{blue!25} 83\%  & \cellcolor{blue!25} 1.90 & \cellcolor{blue!25} 23.37 & \cellcolor{blue!25} 74\%\\
\textsc{Switchboard+OneUtt}  & 6.46          & 362.90  & 28\%   & \cellcolor{blue!25} 1.52            & \cellcolor{blue!25} 15.19 & \cellcolor{blue!25} 78\% & \cellcolor{blue!25} 2.62& \cellcolor{blue!25} 45.06 & \cellcolor{blue!25}68\%\\
\textsc{BERT+OneUtt}      & 7.35          & 494.18    & 4\% & \cellcolor{blue!25} 1.81            & \cellcolor{blue!25}17.34  & \cellcolor{blue!25}75\%   &  \cellcolor{blue!25}2.53 & \cellcolor{blue!25}42.93 & \cellcolor{blue!25}66\%\\
\textsc{CHILDES-1gram}   & 8.79          & 314.09    & 3\%  & \cellcolor{blue!25}2.26            & \cellcolor{blue!25}15.89  & \cellcolor{blue!25}69\%   &  \cellcolor{blue!25}3.76 & \cellcolor{blue!25}49.00 & \cellcolor{blue!25}51\% \\
\textsc{UniformPrior}    & 12.97         & 3998.00 & 0\%      & \cellcolor{blue!25}4.61            & \cellcolor{blue!25}62.50 & \cellcolor{blue!25}32\% & \cellcolor{blue!25}4.87 & \cellcolor{blue!25}138.31 & \cellcolor{blue!25}32\%
\end{tabular}
\end{center}
\footnotesize{\noindent $^\star$ The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ Ranks are taken out of a vocabulary of 7,997 possible words.}
\end{table*}

==> CDL (Arxiv revision 2)/tables/model_surprisal_comparison3.tex <==
\begin{table*}
\tablefont
\caption{Model performance as measured by average surprisal, average rank of transcriber interpretation, and percentage of correct top guesses for word recognition models.
The  left column (``Prior'') reflects the distributions from the word prediction module, \ie before using the child's production to identify the word.
The center and right columns reflect the distributions after integrating information from two variants of the pronunciation module.
The full model is indicated in red, which we expect to best replicate adult interpretations of child speech. 
We compare this with a phonetics-only baseline model, which must recognize words solely on the basis of the acoustic signal produced by the child.
Ablated models  test which information sources are most critical for the full model.
%Average surprisal measures the average negative log probability that the model assigns to the words found by transcribers; lower indicates a closer match to adult listeners.
%Average rank indicates the rank of the transcriber's interpretation among the model's hypotheses  (lower is better, e.g., rank = 2 means that it was the second most probable interpretation under the model).
%Percent top 1-guess is the proportion of words in the test set where the model assigns the highest probability among all words in the vocabulary to the word found by annotators; higher is better.
}
\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|lll||lll|lll}
& \multicolumn{3}{c||}{Prior} & \multicolumn{3}{c|}{Posterior with WFST Likelihood} & \multicolumn{3}{c}{Posterior with Lev. Dist. Likelihood} \\
\cline{2-10}
& Average     & Average       & Correct       & Average    & Average & Correct & Average  & Average & Correct  \\
& Surprisal$^\star$     & Rank$^\ddagger$ & Top  & Surprisal$^\star$ & Rank$^\ddagger$ &
Top & Surprisal$^\star$       & Rank$^\ddagger$ & Top       \\
Language Model Prior             & (bits$^\dagger$)        &    &  Guess  & (bits$^\dagger$) &         &  Guess & (bits$^\dagger$)          &      &  Guess \\ \hline
& & & & \multicolumn{3}{c|}{\cellcolor{red!25} Full Model} & \multicolumn{3}{c}{\cellcolor{blue!25} Ablated Models} \\

\textsc{CDL+Context} & 3.30 & 50.21 & 55\% & \cellcolor{red!25} \textbf{0.63} & \cellcolor{red!25} \textbf{2.41} & \cellcolor{red!25} \textbf{90\%} & \cellcolor{blue!25} 1.15 & \cellcolor{blue!25} 7.89 & \cellcolor{blue!25} 83\%  \\

\textsc{Switchboard+Context} & 4.10          & 110.46   & 49\%   & \cellcolor{blue!25} 0.85            & \cellcolor{blue!25} 4.61 & \cellcolor{blue!25} 87\% &  \cellcolor{blue!25} 1.52  & \cellcolor{blue!25} 13.95  & \cellcolor{blue!25} 78\%     \\

\textsc{CDL+LeftContext}     & 4.23  & 88.3   & 46\%  & \cellcolor{blue!25} 0.86 & \cellcolor{blue!25} 4.88  & \cellcolor{blue!25} 86\%   & \cellcolor{blue!25} 1.54   & \cellcolor{blue!25} 15.58 & \cellcolor{blue!25} 78\%  \\


\textsc{BERT+Context}     & 4.63          & 140.99    & 45\%  & \cellcolor{blue!25} 1.02            & \cellcolor{blue!25} 6.16  & \cellcolor{blue!25} 84\%   & \cellcolor{blue!25} 1.69   & \cellcolor{blue!25} 18.52 & \cellcolor{blue!25} 76\%  \\

\textsc{CDL+OneUtt}  & 5.06          & 124.31  & 36\%   & \cellcolor{blue!25} 1.09            & \cellcolor{blue!25} 7.39 & \cellcolor{blue!25} 83\%  & \cellcolor{blue!25} 1.90 & \cellcolor{blue!25} 23.37 & \cellcolor{blue!25} 74\%\\

\textsc{GPT-2+LeftContext}     & 6.45  & 393.87    & 30\%  & \cellcolor{blue!25} 1.90 & \cellcolor{blue!25} 26.06  & \cellcolor{blue!25} 76\%   & \cellcolor{blue!25} 3.03   & \cellcolor{blue!25} 62.24 & \cellcolor{blue!25} 65\%  \\

\textsc{Switchboard+OneUtt}  & 6.46          & 362.90  & 28\%   & \cellcolor{blue!25} 1.52            & \cellcolor{blue!25} 15.19 & \cellcolor{blue!25} 78\% & \cellcolor{blue!25} 2.62 & \cellcolor{blue!25} 45.06 & \cellcolor{blue!25} 68\%\\

\textsc{BERT+OneUtt}      & 7.35          & 494.18    & 25\% & \cellcolor{blue!25} 1.81            & \cellcolor{blue!25} 17.34  & \cellcolor{blue!25} 75\%   &  \cellcolor{blue!25} 2.53 & \cellcolor{blue!25} 42.93 & \cellcolor{blue!25} 66\%\\		

\textsc{CHILDES 3gram} & 7.81  & 674.79  & 14\%  & \cellcolor{blue!25} 2.43 & \cellcolor{blue!25} 20.51  & \cellcolor{blue!25} 67\%   & \cellcolor{blue!25} 3.56   & \cellcolor{blue!25} 55.65 & \cellcolor{blue!25} 56\%  \\

\textsc{GPT2-OneUtt}     & 7.86  & 532.35    & 17\%  & \cellcolor{blue!25} 2.47  & \cellcolor{blue!25} 40.82  & \cellcolor{blue!25} 72\%   & \cellcolor{blue!25} 3.81   & \cellcolor{blue!25} 94.31 & \cellcolor{blue!25} 60\%  \\

\textsc{CHILDES 3gram + OneUtt}  & 7.94  & 480.75  & 30\%  & \cellcolor{blue!25} 1.81 & \cellcolor{blue!25} 14.54  & \cellcolor{blue!25} 75\%   & \cellcolor{blue!25} 2.73   & \cellcolor{blue!25} 41.37 & \cellcolor{blue!25} 66\%  \\

\textsc{CHILDES-1gram}   & 8.79          & 314.09    & 3\%  & \cellcolor{blue!25}2.26            & \cellcolor{blue!25} 15.89  & \cellcolor{blue!25} 69\%   &  \cellcolor{blue!25} 3.76 & \cellcolor{blue!25} 49.00 & \cellcolor{blue!25} 51\% \\

\textsc{UniformPrior}    & 12.97         & 3998.00 & 0\%      & \cellcolor{green!25} 4.61            & \cellcolor{green!25} 62.50 & \cellcolor{green!25} 32\% & \cellcolor{blue!25} 4.87 & \cellcolor{blue!25} 138.31 & \cellcolor{blue!25} 32\% \\

& & &  & \multicolumn{3}{c}{\cellcolor{green!25} Phonetics-Only Baseline Model} & &  & \\


% \textsc{ModelName}     & prior surprisal  & avg prior rank    & correct top guess  & \cellcolor{blue!25} wfst posterior surprisal bits & \cellcolor{blue!25} wfst avg rank  & \cellcolor{blue!25} wfst percent top guess   & \cellcolor{blue!25} levdist posterior surprisal bits   & \cellcolor{blue!25} levdist avg rank \cellcolor{blue!25} levdist percent top guess  \\




% should be easier to get this into the right format from the notebook  



\end{tabular}
\end{center}
\footnotesize{\noindent $^\star$ The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ Ranks are taken out of a vocabulary of 7,997 possible words.}
\end{table*}


% \textsc{ModelName}     & prior surprisal  & avg prior rank    & correct top guess  & \cellcolor{blue!25} wfst posterior surprisal bits & \cellcolor{blue!25} wfst avg rank  & \cellcolor{blue!25} wfst percent top guess   & \cellcolor{blue!25} levdist posterior surprisal bits   & \cellcolor{blue!25} levdist avg rank \cellcolor{blue!25} levdist percent top guess  \\








==> CDL (Arxiv revision 2)/tables/model_surprisal_comparison4.tex <==
\begin{table*}[h]
\tablefont
\caption{Model performance as measured by average surprisal, average rank of transcriber interpretation, and percentage of correct top guesses for word recognition models.
The  left column (``Prior'') reflects the distributions from the word prediction module, \ie before using the child's production to identify the word.
The center and right columns reflect integrating information from two variants of the pronunciation module.
The full model is indicated in red, which we expect to best replicate adult interpretations of child speech. 
We compare this with a phonetics-only baseline model, which must recognize words solely on the basis of the acoustic signal produced by the child (green).
Ablated models test which information sources are most critical for the full model.
\vspace{-5mm}
%Models are ordered by prior surprisal.
%Average surprisal measures the average negative log probability that the model assigns to the words found by transcribers; lower indicates a closer match to adult listeners.
%Average rank indicates the rank of the transcriber's interpretation among the model's hypotheses  (lower is better, e.g., rank = 2 means that it was the second most probable interpretation under the model).
%Percent top 1-guess is the proportion of words in the test set where the model assigns the highest probability among all words in the vocabulary to the word found by annotators; higher is better.
}
\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|lll||lll|lll}
&  \multicolumn{3}{c||}{Prior} & \multicolumn{6}{c}{Posterior} \\

& \multicolumn{3}{c||}{} & \multicolumn{3}{c|}{Phoneme-Specific Likelihood} & \multicolumn{3}{c}{Edit-Distance Likelihood} \\
\cline{2-10}
& Average     & Average       & Correct       & Average    & Average & Correct & Average  & Average & Correct  \\
& Surprisal$^\star$     & Rank$^\ddagger$ & Top  & Surprisal$^\star$ & Rank$^\ddagger$ &
Top & Surprisal$^\star$       & Rank$^\ddagger$ & Top       \\
Language Model Prior             & (bits$^\dagger$)        &    &  Guess$^\Diamond$  & (bits$^\dagger$) &         &  Guess$^\Diamond$ & (bits$^\dagger$)          &      &  Guess$^\Diamond$ \\ \hline
& & & & \multicolumn{3}{c|}{\cellcolor{red!25} Full Model} & \multicolumn{3}{c}{\cellcolor{blue!25} Ablated Models} \\

\textsc{BERT+CHILDES+Bidirectional} & 2.78 & 30.76 & 60\% & \cellcolor{red!25} \textbf{0.57} & \cellcolor{red!25} \textbf{1.80} & \cellcolor{red!25} \textbf{90\%} & \cellcolor{blue!25} 1.03 & \cellcolor{blue!25} 5.63 & \cellcolor{blue!25} 84\%  \\

\textsc{BERT+Switchboard+Bidirectional} & 3.41          & 49.77   & 54\%   & \cellcolor{blue!25} 0.74            & \cellcolor{blue!25} 3.12 & \cellcolor{blue!25} 88\% &  \cellcolor{blue!25} 1.32  & \cellcolor{blue!25} 9.19  & \cellcolor{blue!25} 81\%     \\

\textsc{BERT+CHILDES+Preceding}     & 3.56  & 61.39   & 52\%  & \cellcolor{blue!25} 0.77 & \cellcolor{blue!25} 3.52  & \cellcolor{blue!25} 88\%   & \cellcolor{blue!25} 1.41   & \cellcolor{blue!25} 11.85 & \cellcolor{blue!25} 80\%  \\


\textsc{BERT+AdultWritten+Bidirectional}     & 4.76          & 91.47    & 39\%  & \cellcolor{blue!25} 1.11            & \cellcolor{blue!25} 6.05  & \cellcolor{blue!25} 83\%   & \cellcolor{blue!25} 1.85   & \cellcolor{blue!25} 18.25 & \cellcolor{blue!25} 73\%  \\

\textsc{BERT+CHILDES+OneUtt}  & 5.02          & 124.52  & 36\%   & \cellcolor{blue!25} 1.18            & \cellcolor{blue!25} 7.61 & \cellcolor{blue!25} 82\%  & \cellcolor{blue!25} 2.05 & \cellcolor{blue!25} 24.35 & \cellcolor{blue!25} 72\%\\


\textsc{BERT+Switchboard+OneUtt}  & 6.33          & 342.27  & 28\%   & \cellcolor{blue!25} 1.60            & \cellcolor{blue!25} 15.84 & \cellcolor{blue!25} 78\% & \cellcolor{blue!25} 2.63 & \cellcolor{blue!25} 44.11 & \cellcolor{blue!25} 67\%\\

\textsc{GPT2+CHILDES+Preceding}     & 6.45  & 396.27    & 29\%  & \cellcolor{blue!25} 2.01 & \cellcolor{blue!25} 25.91  & \cellcolor{blue!25} 75\%   & \cellcolor{blue!25} 3.17   & \cellcolor{blue!25} 66.76 & \cellcolor{blue!25} 63\%  \\

\textsc{BERT+AdultWritten+OneUtt}      & 7.16          & 459.78    & 26\% & \cellcolor{blue!25} 1.90            & \cellcolor{blue!25} 18.74  & \cellcolor{blue!25} 74\%   &  \cellcolor{blue!25} 2.92 & \cellcolor{blue!25} 48.8 & \cellcolor{blue!25} 65\%\\		


\textsc{Trigram+CHILDES} & 7.82  & 679.72  & 14\%  & \cellcolor{blue!25} 2.54 & \cellcolor{blue!25} 21.21  & \cellcolor{blue!25} 65\%   & \cellcolor{blue!25} 3.73   & \cellcolor{blue!25} 57.3 & \cellcolor{blue!25} 54\%  \\

\textsc{GPT2+CHILDES+OneUtt}     & 7.88  & 549.98    & 18\%  & \cellcolor{blue!25} 2.60  & \cellcolor{blue!25} 45.41  & \cellcolor{blue!25} 71\%   & \cellcolor{blue!25} 3.99   & \cellcolor{blue!25} 104.85 & \cellcolor{blue!25} 58\%  \\

\textsc{Trigram+CHILDES+OneUtt}  & 8.04  & 490.70  & 29\%  & \cellcolor{blue!25} 1.93 & \cellcolor{blue!25} 15.29  & \cellcolor{blue!25} 73\%   & \cellcolor{blue!25} 2.89   & \cellcolor{blue!25} 43.39 & \cellcolor{blue!25} 63\%  \\

\textsc{Unigram+CHILDES}   & 8.74          & 305.69    & 3\%  & \cellcolor{blue!25} 2.36 & \cellcolor{blue!25} 16.86  & \cellcolor{blue!25} 66\%   &  \cellcolor{blue!25} 3.91 & \cellcolor{blue!25} 50.79 & \cellcolor{blue!25} 49\% \\

\textsc{UniformPrior}    & 12.97         & 3998.00 & 0\%      & \cellcolor{green!25} 4.13           & \cellcolor{green!25} 49.1 & \cellcolor{green!25} 42\% & \cellcolor{blue!25} 5.16 & \cellcolor{blue!25} 143.26 & \cellcolor{blue!25} 30\% \\

& & &  & \multicolumn{3}{c}{\cellcolor{green!25} Phonetics-Only Baseline Model} & &  & \\

% \textsc{ModelName}     & prior surprisal  & avg prior rank    & correct top guess  & \cellcolor{blue!25} wfst posterior surprisal bits & \cellcolor{blue!25} wfst avg rank  & \cellcolor{blue!25} wfst percent top guess   & \cellcolor{blue!25} levdist posterior surprisal bits   & \cellcolor{blue!25} levdist avg rank \cellcolor{blue!25} levdist percent top guess  \\




% should be easier to get this into the right format from the notebook  



\end{tabular}
\end{center}
\vspace{-3mm}
\footnotesize{\noindent $^\star$ A lower surprisal indicates a better model. The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ A lower average rank indicates a better model. Ranks are taken out of a vocabulary of 7,997 possible words.\\
$^\Diamond$ A higher percentage of correct top guess indicates a better model.
}
\end{table*}


% \textsc{ModelName}     & prior surprisal  & avg prior rank    & correct top guess  & \cellcolor{blue!25} wfst posterior surprisal bits & \cellcolor{blue!25} wfst avg rank  & \cellcolor{blue!25} wfst percent top guess   & \cellcolor{blue!25} levdist posterior surprisal bits   & \cellcolor{blue!25} levdist avg rank \cellcolor{blue!25} levdist percent top guess  \\








==> tables/model_surprisal_comparison.tex <==
\begin{table*}
\caption{Average prior and posterior surprisal and rank of transcriber interpretations on $n = 43,993$ phonetic sequences for sixteen Bayesian spoken word recognition models.
This set reflects crossing eight priors with two likelihoods. 
Lower surprisal and lower rank both indicate a closer match to adult listeners.}

 

\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|ll|ll|ll}
                 & \multicolumn{2}{c|}{Prior} & \multicolumn{2}{c|}{Posterior with WFST Likelihood} & \multicolumn{2}{c}{Posterior with Lev. Dist. Likelihood} \\
\cline{2-7}
                 & Average     & Average       & Average       & Average    & Average       & Average    \\
                 & Surprisal$^\star$     & Rank$^\ddagger$       & Surprisal$^\star$       & Rank$^\ddagger$ & Surprisal$^\star$       & Rank$^\ddagger$        \\
Language Model Prior             & (bits$^\dagger$)        &        & (bits$^\dagger$)          & & (bits$^\dagger$)          &         \\ \hline
\textsc{CDL+Context} & 3.30          & 50.21      & 0.63            & 2.41 & 1.15 & 7.89  \\
\textsc{Switchboard+Context} & 4.10          & 110.46      & 0.85            & 4.61 &  1.52  & 13.95       \\
\textsc{BERT+Context}     & 4.63          & 140.99     & 1.02            & 6.16     & 1.69   & 18.52   \\
\textsc{CDL+OneUtt}  & 5.06          & 124.31     & 1.09            & 7.39   & 1.90 & 23.37\\
\textsc{Switchboard+OneUtt}  & 6.46          & 362.90     & 1.52            & 15.19 & 2.62& 45.06\\
\textsc{BERT+OneUtt}      & 7.35          & 494.18     & 1.81            & 17.34     &  2.53 & 42.93 \\
\textsc{CHILDES-1gram}   & 8.79          & 314.09     & 2.26            & 15.89     &  3.76 & 49.00 \\
\textsc{UniformPrior}    & 12.97         & 3998.00       & 4.61            & 62.50 & 4.87 & 138.31 
\end{tabular}
\end{center}
\footnotesize{\noindent $^\star$ The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ Ranks are taken out of a vocabulary of 7,997 possible words.}
\end{table*}

==> tables/model_surprisal_comparison2.tex <==
\begin{table*}
\tablefont
\caption{Model performance as measured by average surprisal, average rank of transcriber interpretation, and percentage of correct top guesses for word recognition models.
The  left column (``Prior'') reflects the distributions from the word prediction module, \ie before using the child's production to identify the word.
The center and right columns reflect the distributions after integrating information from two variants of the pronunciation module.
The full model is indicated in red, which we expect to best replicate adult interpretations of child speech.
This is the best performing model, as indicated in bold.
Other models represent ablations with respect to this full model. 
%Average surprisal measures the average negative log probability that the model assigns to the words found by transcribers; lower indicates a closer match to adult listeners.
%Average rank indicates the rank of the transcriber's interpretation among the model's hypotheses  (lower is better, e.g., rank = 2 means that it was the second most probable interpretation under the model).
%Percent top 1-guess is the proportion of words in the test set where the model assigns the highest probability among all words in the vocabulary to the word found by annotators; higher is better.
}
\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|lll||lll|lll}
                 & \multicolumn{3}{c||}{Prior} & \multicolumn{3}{c|}{Posterior with WFST Likelihood} & \multicolumn{3}{c}{Posterior with Lev. Dist. Likelihood} \\
\cline{2-10}
                 & Average     & Average       & Correct       & Average    & Average       & Correct & Average  & Average & Correct  \\
                 & Surprisal$^\star$     & Rank$^\ddagger$       &
                 Top  & Surprisal$^\star$       & Rank$^\ddagger$ &
                 Top &
                 Surprisal$^\star$       & Rank$^\ddagger$ & Top       \\
Language Model Prior             & (bits$^\dagger$)        &    &  Guess  & (bits$^\dagger$) &         &  Guess & (bits$^\dagger$)          &      &  Guess \\ \hline
& & & & \multicolumn{3}{c|}{\cellcolor{red!25} Full Model} & \multicolumn{3}{c}{\cellcolor{blue!25} Ablated Models}    \\
\textsc{CDL+Context} & 3.30          & 50.21 & 55\%       & \cellcolor{red!25} \textbf{0.63}            & \cellcolor{red!25}\textbf{2.41} & \cellcolor{red!25} \textbf{90\%} & \cellcolor{blue!25} 1.15 & \cellcolor{blue!25} 7.89 & \cellcolor{blue!25} 83\%  \\
\textsc{Switchboard+Context} & 4.10          & 110.46   & 49\%   & \cellcolor{blue!25} 0.85            & \cellcolor{blue!25} 4.61 & \cellcolor{blue!25}87\% &  \cellcolor{blue!25} 1.52  & \cellcolor{blue!25}13.95  & \cellcolor{blue!25} 78\%     \\
\textsc{BERT+Context}     & 4.63          & 140.99    & 45\%  & \cellcolor{blue!25} 1.02            & \cellcolor{blue!25} 6.16  & \cellcolor{blue!25} 84\%   & \cellcolor{blue!25} 1.69   & \cellcolor{blue!25} 18.52 & \cellcolor{blue!25} 76\%  \\
\textsc{CDL+OneUtt}  & 5.06          & 124.31  & 36\%   & \cellcolor{blue!25} 1.09            & \cellcolor{blue!25} 7.39 & \cellcolor{blue!25} 83\%  & \cellcolor{blue!25} 1.90 & \cellcolor{blue!25} 23.37 & \cellcolor{blue!25} 74\%\\
\textsc{Switchboard+OneUtt}  & 6.46          & 362.90  & 28\%   & \cellcolor{blue!25} 1.52            & \cellcolor{blue!25} 15.19 & \cellcolor{blue!25} 78\% & \cellcolor{blue!25} 2.62& \cellcolor{blue!25} 45.06 & \cellcolor{blue!25}68\%\\
\textsc{BERT+OneUtt}      & 7.35          & 494.18    & 4\% & \cellcolor{blue!25} 1.81            & \cellcolor{blue!25}17.34  & \cellcolor{blue!25}75\%   &  \cellcolor{blue!25}2.53 & \cellcolor{blue!25}42.93 & \cellcolor{blue!25}66\%\\
\textsc{CHILDES-1gram}   & 8.79          & 314.09    & 3\%  & \cellcolor{blue!25}2.26            & \cellcolor{blue!25}15.89  & \cellcolor{blue!25}69\%   &  \cellcolor{blue!25}3.76 & \cellcolor{blue!25}49.00 & \cellcolor{blue!25}51\% \\
\textsc{UniformPrior}    & 12.97         & 3998.00 & 0\%      & \cellcolor{blue!25}4.61            & \cellcolor{blue!25}62.50 & \cellcolor{blue!25}32\% & \cellcolor{blue!25}4.87 & \cellcolor{blue!25}138.31 & \cellcolor{blue!25}32\%
\end{tabular}
\end{center}
\footnotesize{\noindent $^\star$ The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ Ranks are taken out of a vocabulary of 7,997 possible words.}
\end{table*}

==> tables/model_surprisal_comparison3.tex <==
\begin{table*}
\tablefont
\caption{Model performance as measured by average surprisal, average rank of transcriber interpretation, and percentage of correct top guesses for word recognition models.
The  left column (``Prior'') reflects the distributions from the word prediction module, \ie before using the child's production to identify the word.
The center and right columns reflect the distributions after integrating information from two variants of the pronunciation module.
The full model is indicated in red, which we expect to best replicate adult interpretations of child speech. 
We compare this with a phonetics-only baseline model, which must recognize words solely on the basis of the acoustic signal produced by the child.
Ablated models  test which information sources are most critical for the full model.
%Average surprisal measures the average negative log probability that the model assigns to the words found by transcribers; lower indicates a closer match to adult listeners.
%Average rank indicates the rank of the transcriber's interpretation among the model's hypotheses  (lower is better, e.g., rank = 2 means that it was the second most probable interpretation under the model).
%Percent top 1-guess is the proportion of words in the test set where the model assigns the highest probability among all words in the vocabulary to the word found by annotators; higher is better.
}
\label{tab:model_surprisal_comparison}
\begin{center}
\begin{tabular}{l|lll||lll|lll}
& \multicolumn{3}{c||}{Prior} & \multicolumn{3}{c|}{Posterior with WFST Likelihood} & \multicolumn{3}{c}{Posterior with Lev. Dist. Likelihood} \\
\cline{2-10}
& Average     & Average       & Correct       & Average    & Average & Correct & Average  & Average & Correct  \\
& Surprisal$^\star$     & Rank$^\ddagger$ & Top  & Surprisal$^\star$ & Rank$^\ddagger$ &
Top & Surprisal$^\star$       & Rank$^\ddagger$ & Top       \\
Language Model Prior             & (bits$^\dagger$)        &    &  Guess  & (bits$^\dagger$) &         &  Guess & (bits$^\dagger$)          &      &  Guess \\ \hline
& & & & \multicolumn{3}{c|}{\cellcolor{red!25} Full Model} & \multicolumn{3}{c}{\cellcolor{blue!25} Ablated Models} \\

\textsc{CDL+Context} & 3.30 & 50.21 & 55\% & \cellcolor{red!25} \textbf{0.63} & \cellcolor{red!25} \textbf{2.41} & \cellcolor{red!25} \textbf{90\%} & \cellcolor{blue!25} 1.15 & \cellcolor{blue!25} 7.89 & \cellcolor{blue!25} 83\%  \\

\textsc{Switchboard+Context} & 4.10          & 110.46   & 49\%   & \cellcolor{blue!25} 0.85            & \cellcolor{blue!25} 4.61 & \cellcolor{blue!25} 87\% &  \cellcolor{blue!25} 1.52  & \cellcolor{blue!25} 13.95  & \cellcolor{blue!25} 78\%     \\

\textsc{CDL+LeftContext}     & 4.23  & 88.3   & 46\%  & \cellcolor{blue!25} 0.86 & \cellcolor{blue!25} 4.88  & \cellcolor{blue!25} 86\%   & \cellcolor{blue!25} 1.54   & \cellcolor{blue!25} 15.58 & \cellcolor{blue!25} 78\%  \\


\textsc{BERT+Context}     & 4.63          & 140.99    & 45\%  & \cellcolor{blue!25} 1.02            & \cellcolor{blue!25} 6.16  & \cellcolor{blue!25} 84\%   & \cellcolor{blue!25} 1.69   & \cellcolor{blue!25} 18.52 & \cellcolor{blue!25} 76\%  \\

\textsc{CDL+OneUtt}  & 5.06          & 124.31  & 36\%   & \cellcolor{blue!25} 1.09            & \cellcolor{blue!25} 7.39 & \cellcolor{blue!25} 83\%  & \cellcolor{blue!25} 1.90 & \cellcolor{blue!25} 23.37 & \cellcolor{blue!25} 74\%\\

\textsc{GPT-2+LeftContext}     & 6.45  & 393.87    & 30\%  & \cellcolor{blue!25} 1.90 & \cellcolor{blue!25} 26.06  & \cellcolor{blue!25} 76\%   & \cellcolor{blue!25} 3.03   & \cellcolor{blue!25} 62.24 & \cellcolor{blue!25} 65\%  \\

\textsc{Switchboard+OneUtt}  & 6.46          & 362.90  & 28\%   & \cellcolor{blue!25} 1.52            & \cellcolor{blue!25} 15.19 & \cellcolor{blue!25} 78\% & \cellcolor{blue!25} 2.62 & \cellcolor{blue!25} 45.06 & \cellcolor{blue!25} 68\%\\

\textsc{BERT+OneUtt}      & 7.35          & 494.18    & 25\% & \cellcolor{blue!25} 1.81            & \cellcolor{blue!25} 17.34  & \cellcolor{blue!25} 75\%   &  \cellcolor{blue!25} 2.53 & \cellcolor{blue!25} 42.93 & \cellcolor{blue!25} 66\%\\		

\textsc{CHILDES 3gram} & 7.81  & 674.79  & 14\%  & \cellcolor{blue!25} 2.43 & \cellcolor{blue!25} 20.51  & \cellcolor{blue!25} 67\%   & \cellcolor{blue!25} 3.56   & \cellcolor{blue!25} 55.65 & \cellcolor{blue!25} 56\%  \\

\textsc{GPT2-OneUtt}     & 7.86  & 532.35    & 17\%  & \cellcolor{blue!25} 2.47  & \cellcolor{blue!25} 40.82  & \cellcolor{blue!25} 72\%   & \cellcolor{blue!25} 3.81   & \cellcolor{blue!25} 94.31 & \cellcolor{blue!25} 60\%  \\

\textsc{CHILDES 3gram + OneUtt}  & 7.94  & 480.75  & 30\%  & \cellcolor{blue!25} 1.81 & \cellcolor{blue!25} 14.54  & \cellcolor{blue!25} 75\%   & \cellcolor{blue!25} 2.73   & \cellcolor{blue!25} 41.37 & \cellcolor{blue!25} 66\%  \\

\textsc{CHILDES-1gram}   & 8.79          & 314.09    & 3\%  & \cellcolor{blue!25}2.26            & \cellcolor{blue!25} 15.89  & \cellcolor{blue!25} 69\%   &  \cellcolor{blue!25} 3.76 & \cellcolor{blue!25} 49.00 & \cellcolor{blue!25} 51\% \\

\textsc{UniformPrior}    & 12.97         & 3998.00 & 0\%      & \cellcolor{green!25} 4.61            & \cellcolor{green!25} 62.50 & \cellcolor{green!25} 32\% & \cellcolor{blue!25} 4.87 & \cellcolor{blue!25} 138.31 & \cellcolor{blue!25} 32\% \\

& & &  & \multicolumn{3}{c}{\cellcolor{green!25} Phonetics-Only Baseline Model} & &  & \\


% \textsc{ModelName}     & prior surprisal  & avg prior rank    & correct top guess  & \cellcolor{blue!25} wfst posterior surprisal bits & \cellcolor{blue!25} wfst avg rank  & \cellcolor{blue!25} wfst percent top guess   & \cellcolor{blue!25} levdist posterior surprisal bits   & \cellcolor{blue!25} levdist avg rank \cellcolor{blue!25} levdist percent top guess  \\




% should be easier to get this into the right format from the notebook  



\end{tabular}
\end{center}
\footnotesize{\noindent $^\star$ The difference in average probability assigned to the transcriber interpretation is $2^{\text{diff}}$, where $\text{diff}$ is the difference between two model scores. \\
% link to the posteriors
$^\dagger$ Paired \textit{t}-tests yield statistically significant pairwise differences between all model surprisal values, $p<10^{-5}$. \\
%link to the ranks
$^\ddagger$ Ranks are taken out of a vocabulary of 7,997 possible words.}
\end{table*}


% \textsc{ModelName}     & prior surprisal  & avg prior rank    & correct top guess  & \cellcolor{blue!25} wfst posterior surprisal bits & \cellcolor{blue!25} wfst avg rank  & \cellcolor{blue!25} wfst percent top guess   & \cellcolor{blue!25} levdist posterior surprisal bits   & \cellcolor{blue!25} levdist avg rank \cellcolor{blue!25} levdist percent top guess  \\







